Fair Representation Learning using Interpolation Enabled Disentanglement

With the growing interest in the machine learning community to solve real-world problems, it has become crucial to uncover the hidden reasoning behind their decisions by focusing on the fairness and auditing the predictions made by these black-box models. In this paper, we propose a novel method to address two key issues: (a) Can we simultaneously learn fair disentangled representations while ensuring the utility of the learned representation for downstream tasks, and (b)Can we provide theoretical insights into when the proposed approach will be both fair and accurate. To address the former, we propose the method FRIED, Fair Representation learning using Interpolation Enabled Disentanglement. In our architecture, by imposing a critic-based adversarial framework, we enforce the interpolated points in the latent space to be more realistic. This helps in capturing the data manifold effectively and enhances the utility of the learned representation for downstream prediction tasks. We address the latter question by developing a theory on fairness-accuracy trade-offs using classifier-based conditional mutual information estimation. We demonstrate the effectiveness of FRIED on datasets of different modalities - tabular, text, and image datasets. We observe that the representations learned by FRIED are overall fairer in comparison to existing baselines and also accurate for downstream prediction tasks. Additionally, we evaluate FRIED on a real-world healthcare claims dataset where we conduct an expert aided model auditing study providing useful insights into opioid ad-diction patterns.

==> sections/prelimanaries.tex <==
\section{Preliminaries}\label{background}
% \subsection{Intersectional Fairness} 
% The concept of `intersectionality', derived from feminist literature, primarily focuses on viewing humans as a combination of multiple identities such as race, gender, economic status, etc. \cite{bunjun2010feminist}. 
% This can be further extended to the idea of fairness, or its lack thereof, in machine learning models. The seminal work, `Gender Shades' by \citet{buolamwini2018gender} highlights the worrying differences in the error rates for automated facial analysis that stems from the intersectionality of gender and skin color. 
% Despite the pressing need to incorporate multiple identities, most of the work in this field has focused primarily on using a single identity which can be exclusionary. The primary objective of intersectional fairness is to consider multiple protected attributes and incorporate them cohesively into the model to provide a fair solution. We aim to achieve this in our work by semantically combining multiple protected attributes using interpolation (described in detail in Section \ref{method}). Our model performance when compared to the trivial baselines are shown in Section \ref{sec:trivial_baseline}.

% \subsection{Interpolation}
% Interpolation is defined as the convex combination of latent representations of two data points resulting in an output that represents the important semantic properties from input instances \cite{lounsbery1992parametric}. It has been shown that autoencoders can interpolate. For example, one of the recent works, Adversarially Constrained Autoencoder Interpolation (ACAI) \cite{berthelot2018understanding} uses an adversarial regularizer for improving interpolation. 

% In our model, we incorporate interpolation to semantically combine meaningful properties from multiple protected attributes using an interpolation co-efficient, $\alpha$. This helps in learning better representations. Irrespective of the number of input dimensions, it is essential to operate in latent space as that has been shown to generate more realistic data points. It results in a smoother data manifold \cite{berthelot2018understanding} unlike direct interpolation in data space which might not result in smooth morphing of input instances. 
Let $p$ denote the protected attribute, $X$ denote the feature vector, $Y$ denote the true label for the binary classification case and $\hat{Y}$ denote the predicted label. Let $X_k$ denote the feature vector for instances $k$. $X'$ is the representation obtained after interpolation. \textcolor{red}{Describe your notations here. Describe the problem statement.}

%For each group $p=z$, we will be considering classifiers of the form $T_z(x)\overset{H_1}{\geq}\tau_z$, i.e., the prediction label is $\mathbbm{1}(T_z(x)\geq \tau_z)$ where $ \mathbbm{1}(\cdot)$ is the indicator function. Thus, the predicted label for $(X,p)=(x,z)$ is given by:
% \begin{align}
% \hat{Y}(x,z)=\begin{cases}
% \mathbbm{1}(T_0(x)\geq \tau_0), & z=0 \\
% \mathbbm{1}(T_1(x)\geq \tau_1), & z=1.
% \end{cases}\label{eq:classifier}
% \end{align}

% \subsection{Disentangled Representations}\label{back:disent}

% Disentangled representations have gained considerable recognition in the past few years because of their ability to generalize to other tasks, increased interpretability, applicability in several downstream tasks, etc. \cite{locatello2019challenging}. They are essentially an unsupervised learning technique that aim to learn a complete feature independent of other nodes. The benefit of disentangled representations is that the higher level generative features of the data are captured by the disjoint latent codes. These disentangled representations have shown to be fairer with respect to predictions made on downstream tasks \cite{locatello2019fairness} and can also be used to compute the influence of a feature on model outcome. In their recent work, Marx \textit{et al.} \citep{marx2019disentangling} developed a procedure that made use of disentangled representations to identify the indirect influence of one or more features in the dataset. They demonstrated using SHAP plots \cite{lundberg2017unified} that these proxy features helped audit black box models.

